How Should We Support Designing Privacy-Friendly Apps for Children? Using a Research through Design Process to Understand Developers' Needs and Challenges

Mobile apps used by children often make use of harmful techniques, such as data tracking and targeted advertising. Previous research has suggested that developers face several systemic challenges in designing apps that prioritise children's best interests. To understand how developers can be better supported, we used a Research through Design (RtD) method to explore what the future of privacy-friendly app development could look like. We performed an elicitation study with 20 children's app developers to understand their needs and requirements. We found a number of specific technical requirements from the participants about how they would like to be supported, such as having actionable transnational design guidelines and easy-to-use development libraries. However, participants were reluctant to adopt these design ideas in their development practices due to perceived financial risks associated with increased privacy in apps. To overcome this critical gap, participants formulated socio-technical requirements that extend to other stakeholders in the mobile industry, including parents and marketplaces. Our findings provide important immediate and long-term design opportunities for the HCI community, and indicate that support for changing app developers' practices must be designed in the context of their relationship with other stakeholders.

==> contents/introduction.tex <==
\section{Introduction}
The pace at which technological advancements have been made in the past few decades has shifted many children's activities from the physical to the digital. Children are spending more time online through mobile devices now than ever before \cite{ofcom2018children, livingstone2017children, ofcom2018children}. A recent report shows that nearly all children aged 3 - 17 in the UK have been spending time online, primarily through mobile devices such as smartphones (72\%) and tablets (69\%) \cite{britain2022children}, and over 60\% of children under the age of 13 have a social media profile \cite{britain2022children}. Unsurprisingly, the industry for developing, distributing, and monetising services and applications aimed at children is thriving. Mobile marketplaces, such as the Google Play Store and the Apple App Store, all offer specific categories of apps aimed at children \cite{google_expert, apple_arcade, google_play_pass}.

The increased use of mobile applications by children does not come without risks and harms \cite{livingstone2017children}. Data privacy is one such risk, a large portion of which can be attributed to the use of third-party development libraries, which have now become an essential part of mobile app development \cite{balebako2014privacy}. App developers often opt for these libraries for the ease of development, but more often for data monetisation. These libraries are often embedded with data trackers to collect sensitive user data \cite{book2013longitudinal, lin2013understanding, reyes2018won}, including location information, and share processed data with data brokers for analytics purposes. This issue is particularly concerning for children~\cite{binns2018third} as research has shown that ``family apps" are often associated with more trackers than many other app genres \cite{livingstone2017children}. Furthermore, children's understanding of such digital risks is less developed than that of adults \cite{livingstone2017children, lapenta2015youth, emanuel2014exploring, zhao2019make}, raising a critical need \textcolor{blue}{to} explore how we can better support children's privacy rights and autonomy \cite{peter2011adolescents, raynes2014gaming, pradeep2016virtual, balleys2017being}.

Over the past few years, concerns have been expressed by regulatory bodies, human rights organisations, and industry stakeholders that children's privacy and the commercial use of their data \textcolor{blue}{are} at risk \cite{lupton2017datafied}. A notable direction in which efforts have been made to improve the state of privacy for children is by rethinking the role of developers and service providers. For example, the UK Information Commissioner’s Office (ICO) introduced the statutory Age-Appropriate Design Code (AADC) \cite{ico_2020} in 2021, which requires services and applications aimed at children to consider data protection as a key element as part of their design. However, enforcing compliance is not without challenge. For this study, we broadly refer to being \textit{``privacy-friendly''} as the design principles that minimise the amount of implicit personal data collection and sharing in apps through the use of data trackers embedded in third-party app development libraries and advertising modules. We are interested to examine how app developers for children may need to be better supported for building privacy-friendly apps, given the increased legislation developments in the UK.


In recent years, the human-computer interaction (HCI) community has seen growth in research involving app developers. Despite this progress, much of the research has primarily focused on understanding app developers' perceptions and practices \cite{li2021developers, tahaei2021privacy, ekambaranathan2020understanding, mhaidli2019we}. For example, it has been shown that developers often choose SDKs and third-party libraries based on their popularity, rather than considering their potential impacts on user privacy and security \cite{mhaidli2019we, ekambaranathan2021money}. Additionally, app developers frequently maintain default configurations for these tools \cite{tahaei2021developers}, which may not adequately protect users' data. Developers have also been found \textcolor{blue}{to} often lack practical support, for example through guidelines and SDKs, for their implementation of privacy-friendly features, and face systemic monetary constraints placed on them by marketplaces, leading to them having to make a trade-off between sustaining their business and protecting children's privacy \cite{ekambaranathan2020understanding, ekambaranathan2021money}. While all these studies point to the need for usable tools to help app developers, research in this direction is still limited, and few efforts have been made to support them through concrete tools. 

Therefore, in this study we \textcolor{blue}{aim} to understand how these practical and structural challenges can be overcome. We make use of \textcolor{blue}{the} Research through Design (RtD) approach \cite{zimmerman2007research} to explore what future tools could look like \textcolor{blue}{that would} support developers in creating privacy-friendly apps for children. We were guided by the following research questions:

\begin{enumerate}
    \item How do app developers want specific development tools to enable better privacy in children's apps to look like?
    \item What requirements do app developers foresee for tools to support their development of future privacy-friendly apps for children?
    \item How do app developers envision overcoming systemic barriers, imposed by major marketplaces, to creating privacy-friendly apps?
\end{enumerate}

The socio-technical nature and complexity of the challenges we \textcolor{blue}{aim} to address mean that potentially disruptive ideas are needed to overcome the systems currently put in place. For this reason, we made use of an RtD method, which is a co-design methodology that allows researchers to design and discuss ideas \textcolor{blue}{that} may seem futuristic, disruptive and even technically infeasible to realise \cite{stappers2017research}. Using a set of design ideas generated by expert designers, we were able to engage with app developers more effectively, elicit their technological requirements for integrating privacy considerations as a part of the development process. Previous research has shown that RtD is particularly effective for identifying users' latent needs in support of `wicked problems', which can be challenging to design for~\cite{zimmerman2007research,rittel1973dilemmas}. To this end, we performed an ideation workshop with expert designers in which we generated 12 speculative designs aimed at supporting developers in creating privacy-friendly apps. We presented and discussed these designs with 20 children's app developers through semi-structured interviews to elicit their reactions and understand what their requirements are when envisioning the future of privacy-friendly app development.

Our findings confirmed the technical and systemic barriers identified in previous research and identified \textcolor{blue}{specific} thoughts and requirements from our participants regarding how practical tools and guidance should look like. Furthermore, although our results showed that participants were wary \textcolor{blue}{of} addressing systemic challenges through some of the more disruptive ideas we proposed (e.g. through alternative marketplaces), they formulated critical socio-technical barriers that prevent current practice changes and indicated the need for a multi-stakeholder multi-disciplinary approach \textcolor{blue}{to} understanding the interplay of incentives and behaviours of multiple stakeholders, including parents, children, and marketplaces. Our findings provide important implications and opportunities for design, the potential for \textcolor{blue}{changing} power structures in the mobile ecosystem, and key directions for concretely supporting developers.

